Analyzing Code Comments to Boost Program Comprehension

We are trying to find source code comments that help programmers understand a nontrivial part of source code. One of such examples would be explaining to assign a zero as a way to "clear" a buffer. Such comments are invaluable to programmers and identifying them correctly would be of great help. Toward this goal, we developed a method to discover explanatory code comments in a source code. We first propose eleven distinct categories of code comments. We then developed a decision-tree based classifier that can identify explanatory comments with 60% precision and 80% recall. We analyzed 2,000 GitHub projects that are written in two languages: Java and Python. This task is novel in that it focuses on a microscopic comment ("local comment") within a method or function, in contrast to the prior efforts that focused on API- or method-level comments. We also investigated how different category of comments is used in different projects. Our key finding is that there are two dominant types of comments: preconditional and postconditional. Our findings also suggest that many English code comments have a certain grammatical structure that are consistent across different projects.

==> Makefile <==
# Makefile for LaTeX

RM=rm -f
ZIP=zip
GV2SVG=dot -Tsvg
SVG2PDF=rsvg-convert -f pdf
TEX2DVI=pdflatex
DVI2PDF=dvipdfmx
VIEWPDF=mupdf

TARGET=final.pdf

FIGS=fig/biochunk.pdf \
	fig/cat_java.pdf \
	fig/cat_python.pdf \
	fig/decisiontree.pdf \
	fig/javaparse.pdf \
	fig/pipeline.pdf \
	fig/relation.pdf \
	fig/target.pdf \
	fig/screenshot.png

all: $(TARGET)

zip: clean
	$(ZIP) -r all.zip -x'**/.*' fig final.tex *.sty *.cls Makefile

clean:
	-$(RM) *.dvi *.aux *.log *.out *.pdf

view: $(TARGET)
	$(VIEWPDF) $(TARGET)

$(TARGET): $(FIGS)

.SUFFIXES: .gv .svg .pdf .tex .dvi

.gv.svg:
	$(GV2SVG) -o $@ $<
.svg.pdf:
	$(SVG2PDF) -o $@ $<
.tex.dvi:
	$(TEX2DVI) $< && $(TEX2DVI) $< && $(TEX2DVI) $<
.dvi.pdf:
	$(DVI2PDF) $<

